Training a Scientific Reasoning Model for Chemistry

Reasoning models are large language models that emit a long chain-of-thought before answering, providing both higher accuracy and explicit reasoning for their response. A major question has been whether language model reasoning generalizes beyond mathematics, programming, and logic, where most previous work has focused. We demonstrate that reasoning models can be post-trained for chemistry without additional domain pretraining, and require substantially less data compared to contemporary domain-specific models. We report ether0, a 24B parameter LLM (based on Mistral-Small-24B) that can reason in natural language and respond with chemical structures. This reasoning model was trained with reinforcement learning on 640,730 experimentally-grounded chemistry problems across 375 tasks ranging from synthesizability, to blood-brain barrier permeability, to human receptor activity, to scent. Our model exceeds general-purpose chemistry models, frontier models, and human experts on molecular design tasks. It is also more data efficient relative to specialized models. We anticipate that this method can be applied to train data-efficient language models specialized for tasks across a wide variety of scientific domains.

==> datasheet.tex <==
\newpage
\section*{Datasheet for Datasets}

We used the template suggested by \citep{Gebru2018-bd} to document our dataset creation.

\subsection*{MOTIVATION}

    \textbf{For what purpose was the dataset created?}\\
    %%%
    Our study focus on training a generalist reasoning model for chemistry. Hence, our model needs to be trained on multiple tasks. There is no such multi-problem dataset. Our dataset is a curation of several available task-specific datasets.
    %%% 
    
    \textbf{Who created this dataset (e.g., which team, research group) and on behalf entity (e.g., company, institution, organization)?} \\
    %%%
    The dataset was put together and curated by the authors.\\
    %%% 
    
    \textbf{What support was needed to make this dataset?}\\
    %%%
    No additional support was needed. All tasks considered in our study are available in open-source datasets.\\
    %%% 
    
    \textbf{Any other comments?} \\
    %%%
    No.
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{COMPOSITION}
    \textbf{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)?}\\
    %%%
    Every task in the dataset is a common chemistry problem. Examples are: string representation of molecules completion, chemistry multiple-choice questions, molecular functional groups prediction, etc. The whole dataset is composed of natural language textual content only. \\
    %%% 
    
    \textbf{How many instances are there in total (of each type, if appropriate)?} \\
    %%%
    The dataset is composed of 577790 questions. See~\autoref{tab:tasks} for information about each task.\\
    %%% 
    
    \textbf{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?}\\
    %%%
    It is a sample of multiple instances. The number of examples on each instance is available in~\autoref{tab:tasks}, and the sampling strategy is available in~\autoref{sec:dataset}. \\
    %%% 
    
    \textbf{What data does each instance consist of?}\\
    %%%
    The dataset consists of chemistry-related questions and answers.\\
    %%% 
    
    \textbf{Is there a label or target associated with each instance?}\\
    %%%
    Some of the questions are multiple-choice questions, which have an expected correct answer. Other questions have a target answer that can be used to verify the model's response. \\
    %%% 
    
    \textbf{Is any information missing from individual instances?}\\
    %%%
    No. Some questions exhibit partial (consequently invalid) SMILES strings, as the goal of the task is to complete the string with a valid molecule. However, the original molecule used to generate the question is distributed together with each instance.\\
    %%% 
    
    \textbf{Are relationships between individual instances made explicit (e.g., users’movie ratings, social network links)?}\\
    %%%
    N/A. \\
    %%% 
    
    \textbf{Are there recommended data splits (e.g., training, development/validation, testing)?}\\
    %%%
    Yes. The dataset is distributed in a HuggingFace repository with a recommended data split.\\
    %%% 
    
    \textbf{Are there any errors, sources of noise, or redundancies in the dataset?}\\
    %%%
    No. \\
    %%% 
    
    \textbf{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g., websites, tweets, other datasets)?} \\
    %%%
    Our dataset is self-contained. We host and distribute it independently despite being curated from other open-source datasets. Reference for the original datasets are available in~\autoref{tab:tasks} \\
    %%% 
    
    \textbf{Does the dataset contain data that might be considered confidential (e.g., data that is protected by legal privilege or by doctor-patient confidentiality, data that includes the content of individuals’ non-public communications)?}\\
    %%%
    No. \\
    %%% 
    
    \textbf{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?}\\
    %%%
    No. \\
    %%% 
    
    \textbf{Does the dataset relate to people?}\\
    %%%
    No. \\
    %%% 
    
    \textbf{Does the dataset identify any subpopulations (e.g., by age, gender)?} \\
    %%%
    N/A \\
    %%% 
    
    \textbf{Is it possible to identify individuals (i.e., one or more natural persons), either directly or indirectly (i.e., in combination with other data) from the dataset?}\\
    %%%
    N/A \\
    %%% 
    
    \textbf{Does the dataset contain data that might be considered sensitive in any way (e.g., data that reveals racial or ethnic origins, sexual orientations, religious beliefs, political opinions or union memberships, or locations; financial or health data; biometric or genetic data; forms of government identification, such as social security numbers; criminal history)?} \\
    %%%
    N/A \\
    %%% 
    
    \textbf{Any other comments?}\\
    %%%
    No. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{COLLECTION}

    \textbf{How was the data associated with each instance acquired?}\\
    %%%
    The data was obtained from other open-source datasets and curated by the authors.\\
    %%% 
    
    \textbf{Over what timeframe was the data collected?}\\
    %%%
    The dataset was built over the course of the project. There were no timeframe in which 100\% of the time was dedicated to the project creation. \\
    %%% 
    
    \textbf{What mechanisms or procedures were used to collect the data (e.g., hardware apparatus or sensor, manual human curation, software program, software API)?
    }\\
    %%%
    A complete description of the dataset curation is available in~\autoref{sec:dataset}. \\
    %%% 
    
    \textbf{What was the resource cost of collecting the data?}\\
    %%%
    We did not evaluate the cost of the data collection. \\
    %%% 
    
    \textbf{If the dataset is a sample from a larger set, what was the sampling strategy (e.g., deterministic, probabilistic with specific sampling
    probabilities)?}\\
    %%%
    A complete description of the dataset curation is available in~\autoref{sec:dataset}. \\
    %%% 
    
    \textbf{Who was involved in the data collection process (e.g., students, crowdworkers, contractors) and how were they compensated (e.g., how much were crowdworkers paid)?}\\
    %%%
    The authors were responsible for collecting and curating the dataset. \\
    %%% 
    
    \textbf{Were any ethical review processes conducted (e.g., by an institutional review board)?}\\
    %%%
    No. \\
    %%% 
    
    \textbf{Does the dataset relate to people?} \\
    %%%
    No. \\
    %%% 
    
    \textbf{Did you collect the data from the individuals in question directly, or obtain it via third parties or other sources (e.g., websites)?}\\
    %%%
    N/A \\
    %%% 
    
    \textbf{Were the individuals in question notified about the data collection?}\\
    %%%
    N/A \\
    %%% 
    
    \textbf{Did the individuals in question consent to the collection and use of their data?}\\
    %%%
    N/A \\
    %%% 
    
    \textbf{If consent was obtained, were the consenting individuals provided with a mechanism to revoke their consent in the future or for certain uses?}\\
    %%%
    N/A \\
    %%% 
    
    \textbf{Has an analysis of the potential impact of the dataset and its use on data subjects (e.g., a data protection impact analysis) been conducted?} \\
    %%%
    No. \\
    %%% 
    
    \textbf{Any other comments?}\\
    %%%
    No. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{PREPROCESSING / CLEANING / LABELING}

    \textbf{Was any preprocessing/cleaning/labeling of the data
    done (e.g.,discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)?
    }\\
    %%%
    The authors implemented the curation pipeline to generate the chemistry-related questions and answers from the data collected from the open-source datasets. \\
    %%%

    \textbf{Was the ``raw'' data saved in addition to the preprocessed/cleaned/labeled data (e.g., to support unanticipated future uses)?}\\
    %%%
    The ``raw'' data is available in our sources. See~\autoref{tab:tasks} and \autoref{sec:dataset}\\
    %%%

    \textbf{Is the software used to preprocess/clean/label the instances available?}\\
    %%%
    The authors implemented the entire data curation and cleaning process using Python scripts. \\
    %%%

    \textbf{Any other comments?}\\
    %%%
    No. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{USES}

    \textbf{Has the dataset been used for any tasks already?}\\
    %%%
    Yes. This data was used to train the model described in the manuscript. \\
    %%%

    \textbf{Is there a repository that links to any or all papers or systems that use the dataset?}\\
    %%%
    No. This is the first usage of this dataset.\\
    %%%

    \textbf{What (other) tasks could the dataset be used for?}\\
    %%%
    As a chemistry question and answer dataset, we do not anticipate any other uses. The dataset can be used for training and evaluating LLMs. \\
    %%%

    \textbf{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?}\\
    %%%
    No. \\
    %%%

    \textbf{Are there tasks for which the dataset should not be used?}\\
    %%%
    No. \\
    %%%

    \textbf{Any other comments?}\\
    %%%
    No. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{DISTRIBUTION}

    \textbf{
    Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?
    }\\
    %%%
    Yes. The dataset will be public.\\
    %%%

    \textbf{How will the dataset will be distributed (e.g., tarball on website, API, GitHub)?}\\
    %%%
    Yes. It will be distributed as a HuggingFace repository. A DOI will be generated for it. \\
    %%%

    \textbf{When will the dataset be distributed?}\\
    %%%
    The dataset will be released together with the project's code and model upon publication. \\
    %%%

    \textbf{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?}
     \\
    %%%
    The dataset will be distributed under a CC BY license. \\
    %%%

    \textbf{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?}\\
    %%%
    No. \\
    %%%

    \textbf{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?}\\
    %%%
    No. \\
    %%%

    \textbf{Any other comments?}\\
    %%%
    No. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{MAINTENANCE}

    \textbf{Who is supporting/hosting/maintaining the dataset?}\\
    %%%
    The dataset is hosted on HuggingFace and the authors are responsible for maintaining it. \\
    %%%

    \textbf{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}\\
    %%%
    Professional emails are available in the publication and HuggingFace profiles are available in the dataset page.\\
    %%%

    \textbf{Is there an erratum?}\\
    %%%
    No. \\
    %%%

    \textbf{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)?}\\
    %%%
    Yes. The dataset and the project are still in development and will be maintained.\\
    %%%

    \textbf{If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances (e.g., were individuals in question told that their data would be retained for a fixed period of
    time and then deleted)?}\\
    %%%
    N/A \\
    %%%

    \textbf{Will older versions of the dataset continue to be
    supported/hosted/maintained?}\\
    %%%
    N/A \\
    %%%

    \textbf{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?}\\
    %%%
    No external contributions will be allowed to maintain the quality of the dataset. \\
    %%%

    \textbf{Any other comments?}\\
    %%%
    No.
    %%%
